Top-K Maximum Intensity Projection Priors for 3D Liver Vessel Segmentation

Liver-vessel segmentation is an essential task in the pre-operative planning of liver resection. State-of-the-art 2D or 3D convolution-based methods focusing on liver vessel segmentation on 2D CT cross-sectional views, which do not take into account the global liver-vessel topology. To maintain this global vessel topology, we rely on the underlying physics used in the CT reconstruction process, and apply this to liver-vessel segmentation. Concretely, we introduce the concept of top-k maximum intensity projections, which mimics the CT reconstruction by replacing the integral along each projection direction, with keeping the top-k maxima along each projection direction. We use these top-k maximum projections to condition a diffusion model and generate 3D liver-vessel trees. We evaluate our 3D liver-vessel segmentation on the 3D-ircadb-01 dataset, and achieve the highest Dice coefficient, intersection-over-union (IoU), and Sensitivity scores compared to prior work.

==> Paper/method_old.tex <==
\section{Methods}
\label{sec:method}

The proposed \model{} mimics the CT reconstruction\cite{b17} process to correlate the \textsl{msMIP} with the 3D vessel topology. The following sections provide details of our method.

\begin{figure*}
    \centering
    \includegraphics[width=.95\textwidth]{Images/network.pdf}
    \caption{
    \textbf{Architecture of our proposed \model{} model}.
    }
    \label{Figure:network}  % Label changed to match the \fig command
\end{figure*}


\subsection{Vessel graph preparation}
The $3$D vessel graph, which consists of node coordinates and edges between nodes, can be computed based on the $3$D binary liver vessel tree. The $3$D vessel mask is separated into multiple $3$D sub-masks to find their central point coordinates of vessel region, then the edges between nodes are obtained based on the geodesic distance calculation\cite{b22}.

\subsection{msMIP conditioning latent diffusion model}
\model{}, as shown in \fig{network}, employs the latent diffusion model \cite{b19} as the generative part and designs a custom conditional part with GATv2\cite{b21} to ensure the determinants of the liver vessel \textsl{IPs} generation. Latent vessel \textsl{IPs} is generated by a pre-trained KL divergence auto-encoder which is the same as that in LDM\cite{b19}, so we will not provide further demonstrations here.

The forward process of our \model{} is similar to LDM\cite{b19}, Gaussian noise is added to $\mathbf{x}_0$ (latent vessel \textsl{IPs}) given a condition $\mathbf{c}$ (\textsl{msMIP}) from timestep $0$ to \textsl{T}.
The difference between our \model{} and LDM is that we use the time-dependent condition $\mathbf{f}^t=\mathbf{f}_c^t+\mathbf{f}_p^t$ to further constrain the LDM in both training and inference, where $\mathbf{f}_c^t$ is the feature extracted from \textsl{msMIP} and $\mathbf{f}_p^t$ is the projected node embedding computed by GATv2. 

In the reverse process of \model{}, given the condition $\mathbf{f}^t$, the input Gaussian noise $\mathbf{x}_T$ is gradually denoised to the clean liver vessel \textsl{IPs} at timestep $0$, 
represented as:
\begin{align}
    p_{\theta}(\mathbf{x}_{t-1} | \mathbf{x}_t) &= \mathcal{N}(\mathbf{x}_{t-1}; \mu_{\theta}(\mathbf{x}_t | \mathbf{f}^t, t), \sigma) 
    \label{eq:1}
\end{align}

\subsection{Projected node embedding}
$\mathbf{f}_p^t$ provides projected vessel topology at $\mathbf{v}$ to LDM to help the model learn the liver vessel connectivity. 
$\mathbf{f}_p^t$ is represented as:
\begin{align}
    \mathbf{f}_p^t = FP(GAT_{v2}(BP(\mathbf{f}_s^{t,\mathbf{v}})))
    \label{eq:2}
\end{align} 
where $FP(.)$ and $BP(.)$ are the forward and back projection pytorch modules through which the gradient can flow. 
$\mathbf{v}$ contains the views (${...,v_i,v_{i+\alpha},v_{i+2\alpha},...}$) of the \textsl{IPs}, the view interval is $\alpha$.
$\mathbf{f}_s^{t,\mathbf{v}}$ is the sampled node feature at $\mathbf{v}$ at $t$.

Without the $\mathbf{f}_p^t$ as the part of the condition $\mathbf{f}^t$, the model can only generate \textsl{IPs} with replicated vessel structures that were seen in the training set. The following ablation study confirms this.
Therefore, $\mathbf{f}_p^t$ is essential for both the training and inference of the proposed \model{}.
To obtain $\mathbf{f}_p^t$, the node coordinate based $\mathbf{f}_s^{t,\mathbf{v}}$ must be known as (\ref{eq:2}) shows. 
In training, the node coordinates can be calculated based on the binary liver vessel mask.
Since the vessel mask is unknown in inference, we use uniform coordinates to approximate the real coordinates. 
The sampled node feature $\mathbf{f}_s^{t,\mathbf{v}}$ in (\ref{eq:2}) is represented as:
\begin{align}
    \mathbf{f}_s^{t,\mathbf{v}} = GridSample(\mathbf{f}_d^t, coords)
    \label{eq:3}
\end{align}
where $GridSample(.)$ is a coordinate-based sampler, $\mathbf{f}_d^t$ is the time-dependent features extracted by the LDM encoder (first blue block) shown in \fig{network}. 

\subsection{Loss function}
The loss of the \model{} consists of the noise loss and the node loss as shown in \fig{network} and can be written as:
\begin{align}
    Loss &= \arg\min_{x_0}\; ||\epsilon_\theta(x_t|f^t,t)-\epsilon||_2^2 \\ \nonumber
      &\,+ \mathbf{\omega} \cdot (\mathbf{y} \cdot \log(\mathbf{g}) + (1-\mathbf{y}) \cdot \log(1-\mathbf{g}))
    \label{eq:4}
\end{align}
where $\epsilon_\theta(\cdot)$ is modeled by the LDM (the blue blocks in \fig{network}, $\epsilon$ is the Gaussian noise, $\textbf{y}$ are the target node classes ($0$:background, $1$:vessel), $\textbf{g}=GAT_{v2}(BP(\mathbf{f}_s^{t,\mathbf{v}}))$ are the predicted node embeddings, and $\mathbf{\omega}$ is a weight to balance the node classes and we set it to $vessel:background=10:1$ in this study.

\subsection{Post processing}
The consistency between the projections is difficult for the neural network to learn well. 
Minor inconsistencies in the projection domain would cause severe stripe artifacts on the reconstructed images. 
Therefore, we use regularization optimization to suppress these artifacts directly. 
The optimization is represented as:
\begin{align}
    \arg\min_{I} \;  \|A \cdot I - \mathbf{p}\|_2^2
    \label{eq:5}
\end{align}
where $\textsl{A}$ is the system matrix recording the voxel indices penetrated by rays of different projection views, $\mathbf{p}$ are the predicted vessel $\textsl{IPs}$, and $\textsl{I}$ is the optimized object which is initialized by original CT image.
In this study, performing the optimization in (\ref{eq:5}) five times is enough to suppress the stripe artifacts.
To remove small noise spots surrounding the segmented vessel tree, we also perform connected region analysis to cancel them.
